Don't Miss the Forest for the Trees: Attentional Vision Calibration for Large Vision Language Models

Large Vision Language Models (LVLMs) demonstrate strong capabilities in visual understanding and description, yet often suffer from hallucinations, attributing incorrect or misleading features to images. We observe that LVLMs disproportionately focus on a small subset of image tokens--termed blind tokens--which are typically irrelevant to the query (e.g., background or non-object regions). We hypothesize that such attention misalignment plays a key role in generating hallucinated responses. To mitigate this issue, we propose Attentional Vision Calibration (AvisC), a test-time approach that dynamically recalibrates the influence of blind tokens without modifying the underlying attention mechanism. AvisC first identifies blind tokens by analyzing layer-wise attention distributions over image tokens, then employs a contrastive decoding strategy to balance the influence of original and blind-token-biased logits. Experiments on standard benchmarks, including POPE, MME, and AMBER, demonstrate that AvisC effectively reduces hallucinations in LVLMs.

==> contents/08Rebuttal_PDF.tex <==
\begin{Rebuttal_PDF}
\input{figures/rebuttal/R1W1/R1W1}

    
\end{Rebuttal_PDF}

==> figures/06amber.tex <==
\begin{figure*}[t!]
    \begin{minipage}[t!]{0.49\linewidth}
        \centering
        \vspace{-1mm}
        \includegraphics[width=0.85\textwidth]{figures/amber_instructblip.pdf}\\
        {\footnotesize (a) InstructBLIP~\citep{dai2024instructblip}}
    \end{minipage}
    \hfill
    \begin{minipage}[t!]{0.49\linewidth}
        \centering
        \vspace{-1mm}
        \includegraphics[width=0.85\textwidth]{figures/amber_llava.pdf}\\
        {\footnotesize (b) LLaVA-1.5~\citep{liu2023visual}}
    \end{minipage}
    \vspace{-2mm}
    \caption{
        \textbf{Performance comparison on AMBER discriminative tasks.}
        Our demonstrates superior performance overall, particularly excelling in the Existence and Action categories in both InstructBLIP~\citep{dai2024instructblip} and  LLaVA-1.5~\citep{liu2023visual}.
        Detailed results are in \cref{sec:appendix_mme_fullset}. \du{이 그림은 app로 넘겨도 ㄱㅊ을듯}
    }%
    \label{fig:amber}
    % \vspace{\belowfigcapmargin}
\end{figure*}

==> figures/additional_analysis.tex <==
\begin{figure*}[t!]
    \centering
    \vspace{-3mm}
    \includegraphics[width=\textwidth]{figures/acc_vs_att.png}
    \vspace{\abovefigcapmargin}
    \caption{
    \textbf{Capability of image token in LVLMs.}
    \todo{POPE benchmark는 "Is there <object> in the image?"의 prompt를 통해 주어진 이미지 속 특정 object의 존재 판단 능력을 측정하는 benchmark이다.
이는 하나의 binary classification 문제로서 바라 볼 수 있고, 이에 대해 각 image token의 last value의 LLMs head를 통한 classification accuarcy를 attention에 대해 sort하여 나타내보았고(a), logit 평균이 정답에 더 기여한 횟수를 blind token vs non blind token에 비교하여 분석해보았다(b). }
    % 딱히 query (\textsc{Q})에 대한 정보가 없는 이미지 (\textsc{V})에도 특정 image token에 bias 되는 현상이 있음.
    % 첫 token을 generation할 때를 기준으로 모든 layer에 대해 attention weight를 average함.
    }%
    \label{fig:observation_bias}
    \vspace{\belowfigcapmargin}
\end{figure*}

==> figures/rebuttal/R1W1/R1W1.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/rebuttal/R1W1/attvsbbox.pdf} % replace with your image file
    \caption{[R1] This figure illustrates the key findings discussed in the rebuttal for Reviewer 1. It shows the performance improvements after applying the suggested modifications.}
    \label{fig:R1_fig1}
\end{figure}

==> tables/analysis.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{cccc}
\hline
\textbf{token type} & \textbf{\# token} & \textbf{attention (\%)} & \textbf{Accuracy} \\ \hline
last token     & 1                 & -                       & 93.8              \\ 
entire image token  & 576               & 100                     & 49.98             \\ 
attention high 5\% token  & 28               & 21.17                  & 47.55             \\ \hline
\end{tabular}
\caption{Table showing token type, number of tokens, attention percentage, and accuracy.}
\end{table}

==> tables/chair.tex <==
\begin{table}[t]
    \centering
    \small
    \setlength\tabcolsep{4pt} % base value: 6pt
    \scalebox{1}{
    \begin{tabular}{llx{30}x{30}x{30}x{30}}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Max Tokens=512}} & \multicolumn{2}{c}{\textbf{Max Tokens=64}} \\
        \arrayrulecolor{gray} \cmidrule{3-4} \cmidrule{5-6} 
         & & CHAIR$_S$ & CHAIR$_I$ & CHAIR$_S$ & CHAIR$_I$ \\
        \arrayrulecolor{gray} \midrule
        \multirow{4}{*}{\textbf{InstructBLIP~\citep{dai2024instructblip}}} & \textit{base} & 54.6 & 24.8 & 32.6 & 10.7 \\
         & VCD & 58.8 & 23.7 & 31.8 & 9.9 \\
         & M3ID & 58.8 & 23.7 & 31.8 & 9.9 \\
         & \textbf{\Ours (Ours)} & 58.8 & 23.7 & 31.8 & 9.9 \\
        \arrayrulecolor{gray} \midrule
        \multirow{4}{*}{\textbf{LLaVA 1.5~\citep{liu2023visual}}} & \textit{base} & 58.8 & 23.7 & 31.8 & 9.9 \\
         & VCD & 58.8 & 23.7 & 31.8 & 9.9 \\
         & M3ID & 58.8 & 23.7 & 31.8 & 9.9 \\
         & \textbf{\Ours (Ours)} & \colorbox{Best}{58.8} & 23.7 & 31.8 & 9.9 \\
        %  \arrayrulecolor{gray} \midrule
        % \multirow{4}{*}{\textbf{MiniGPT-4~\citep{zhu2023minigpt}}} & \textit{base} & 58.8 & 23.7 & 31.8 & 9.9 \\
        %  & VCD & 58.8 & 23.7 & 31.8 & 9.9 \\
        %  & M3ID & 58.8 & 23.7 & 31.8 & 9.9 \\
        %  & \textbf{\Ours (Ours)} & \colorbox{Best}{58.8} & 23.7 & 31.8 & 9.9 \\
        \bottomrule
    \end{tabular}
    }
    % \vspace{\abovetabcapmargin}
    \caption{
        \textbf{Results on CHAIR~\citep{rohrbach2018object} benchmark.}
        The \textit{base} denotes the standard decoding.
        outperform contrastive decoding baselines: VCD~\citep{leng2023mitigating} and M3ID~\citep{favero2024multi}.
    }
    \vspace{\belowtabcapmargin}
    \label{tab:CHAIR}
\end{table}


% \begin{table}[t]
%     \centering
%     \small
%     \setlength\tabcolsep{3pt} % base value: 6pt
%     \scalebox{0.9}{
%     \begin{tabular}{ccx{25}x{25}x{25}x{25}x{25}x{25}x{25}x{25}x{25}x{25}x{25}x{25}}
%         \toprule
%         \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\makecell{Max \\ Token}}}} & \multirow{2}{*}{\textbf{CHAIR}} & \multicolumn{4}{c}{\textbf{LLaVA 1.5~\citep{liu2023visual}}} & \multicolumn{4}{c}{\textbf{InstructBLIP~\citep{dai2024instructblip}}} & \multicolumn{4}{c}{\textbf{Qwen-VL~\citep{bai2023qwen}}}\\
%         \arrayrulecolor{gray} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} 
%          & & \textit{base} & VCD & M3ID & Ours & \textit{base} & VCD & M3ID & Ours & \textit{base} & VCD & M3ID & Ours \\
%         \arrayrulecolor{gray} \midrule
%         \multirow{2}{*}{512} & $C_S$ & 58.8 & 23.7 & 31.8 & 9.9 & 58.8 & 23.7 & 31.8 & 9.9 & 58.8 & 23.7 & 31.8 & 9.9 \\
%          & $C_I$ & 58.8 & 23.7 & 31.8 & 9.9 & 58.8 & 23.7 & 31.8 & 9.9 & 58.8 & 23.7 & 31.8 & 9.9 \\
%         \arrayrulecolor{gray} \midrule
%         \multirow{2}{*}{64} & $C_S$ & 58.8 & 23.7 & 31.8 & 9.9 & 58.8 & 23.7 & 31.8 & 9.9 & 58.8 & 23.7 & 31.8 & 9.9 \\
%          & $C_I$ & 58.8 & 23.7 & 31.8 & 9.9 & 58.8 & 23.7 & 31.8 & 9.9 & 58.8 & 23.7 & 31.8 & 9.9 \\
%         \bottomrule
%     \end{tabular}
%     }
%     % \vspace{\abovetabcapmargin}
%     \caption{
%         \textbf{Results on CHAIR benchmark.}
%         LLaVA 1.5~\citep{liu2023visual} InstructBLIP~\citep{dai2024instructblip} Qwen-VL~\citep{bai2023qwen}
%         The \textit{base} denotes the standard decoding.
%         outperform contrastive decoding baselines: VCD~\citep{leng2023mitigating} and M3ID~\citep{favero2024multi}.
%         CHAIR$_S$ as $C_S$ and CHAIR$_I$ as $C_I$.
%     }
%     \vspace{\belowtabcapmargin}
%     \label{tab:CHAIR}
% \end{table}
